Finding sparse induced subgraphs on graphs of bounded induced matching treewidth

The induced matching width of a tree decomposition of a graph $G$ is the cardinality of a largest induced matching $M$ of $G$, such that there exists a bag that intersects every edge in $M$. The induced matching treewidth of a graph $G$, denoted by $\mathsf{tree-}\mu(G)$, is the minimum induced matching width of a tree decomposition of $G$. The parameter $\mathsf{tree-}\mu$ was introduced by Yolov [SODA '18], who showed that, for example, Maximum-Weight Independent Set can be solved in polynomial-time on graphs of bounded $\mathsf{tree-}\mu$. Lima, Milani\v{c}, Mur\v{s}i\v{c}, Okrasa, Rz\k{a}\.zewski, and \v{S}torgel [ESA '24] conjectured that this algorithm can be generalized to a meta-problem called Maximum-Weight Induced Subgraph of Bounded Treewidth, where we are given a vertex-weighted graph $G$, an integer $w$, and a $\mathsf{CMSO}_2$-sentence $\Phi$, and are asked to find a maximum-weight set $X \subseteq V(G)$ so that $G[X]$ has treewidth at most $w$ and satisfies $\Phi$. They proved the conjecture for some special cases, such as for the problem Maximum-Weight Induced Forest. In this paper, we prove the general case of the conjecture. In particular, we show that Maximum-Weight Induced Subgraph of Bounded Treewidth is polynomial-time solvable when $\mathsf{tree-}\mu(G)$, $w$, and $|\Phi|$ are bounded. The running time of our algorithm for $n$-vertex graphs $G$ with $\mathsf{tree} - \mu(G) \le k$ is $f(k, w, |\Phi|) \cdot n^{O(k w^2)}$ for a computable function $f$.

==> Preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}
\pdfoutput=1

\usepackage{microtype}
\usepackage[T1]{fontenc}
\usepackage{mdframed}
\usepackage{csquotes}
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}
\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amssymb}
\usepackage{textpos}
\usepackage{amstext}
\usepackage{graphicx,tikz-cd}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{todonotes}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{makecell}
\usepackage{thmtools, thm-restate}
\usepackage{thm-autoref}
 \usepackage{mathdots}
%\usepackage{wrapfig}
\usepackage{multirow}
%\usetikzlibrary{cd}
\usepackage{chngcntr}
\usepackage{apptools}
\usepackage{accents}
\AtAppendix{\counterwithin{lemma}{section}}


 
 \usetikzlibrary{calc}
 \usetikzlibrary{shapes}
 
 \usepackage{tcolorbox} 
\usepackage{xifthen}

\overfullrule=1mm


\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\numberwithin{equation}{section}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{hypothesis}[equation]{Hypothesis}
\newtheorem{claim}[equation]{Claim}
\newtheorem{definition}[equation]{Definition}
\newtheorem{observation}[equation]{Observation}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{mainlemma}[equation]{Main lemma}
%\newtheorem{redrule}[lemma]{Reduction Rule}
%\newtheorem{remark}[lemma]{Remark}
%\newtheorem{reduction}[lemma]{Reduction Rule}
%\newtheorem{conjecture}[lemma]{Conjecture}
\newcommand{\cqed}{\ensuremath{\lhd}}
\makeatletter
\newenvironment{claimproof}{\par
  \pushQED{\cqed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item\relax
  {\itshape
    Proof of the claim\@addpunct{.}}\hspace\labelsep\ignorespaces
}{%
  \hfill\popQED\endtrivlist\@endpefalse
}
\makeatother


\date{}


\usepackage{booktabs}

\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hypertexnames = false,
                 hyperfigures
                 ]{hyperref}

\usepackage[nameinlink]{cleveref}
\crefname{observation}{Observation}{Observations}
\crefname{claim}{Claim}{Claims}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\crefname{mainlemma}{Main lemma}{Main lemmas}




\newcommand{\OO}{\mathcal{O}}
\DeclareMathOperator{\polylog}{polylog}

\newcommand{\CMSO}{\mathsf{CMSO}}

\newcommand{\mwisbt}{\textsc{Maximum-Weight Induced Subgraph of Bounded Treewidth}\xspace}
\newcommand{\mwis}{\textsc{Maximum-Weight Independent Set}\xspace}
\newcommand{\mwif}{\textsc{Maximum-Weight Induced Forest}\xspace}
\newcommand{\treemu}{\mathsf{tree} \textnormal{-} \mu}
\newcommand{\treealpha}{\mathsf{tree} \textnormal{-} \alpha}
\newcommand{\bag}{\mathsf{bag}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\tw}{\mathsf{tw}}
\newcommand{\isfam}{\mathcal{I}}
\newcommand{\bfam}{\mathcal{B}}
\newcommand{\sig}{\mathcal{S}}
\newcommand{\state}{\sigma}
\newcommand{\reps}{\mathcal{R}}
\newcommand{\subtree}{\mathsf{subtree}}
\newcommand{\fami}{\mathcal{F}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\we}{\mathsf{we}}
\newcommand{\vbag}{\mathsf{ibag}}

\newcommand{\topnode}{\mathsf{top}}
\newcommand{\topv}{\mathsf{topv}}

\newcommand{\autom}{\mathcal{A}}
\newcommand{\evaltime}{\mathsf{ET}}
\newcommand{\transit}{\sigma}
\newcommand{\sign}{\mathsf{sign}}
\newcommand{\run}{\rho}



%%%%%%%%%%%%
%%%%% BEGIN FELIX %%%%%%%%%%%%

\newlength{\RoundedBoxWidth}
\newsavebox{\GrayRoundedBox}
\newenvironment{GrayBox}[1]%
{\setlength{\RoundedBoxWidth}{.93\textwidth}
	\def\boxheading{#1}
	\begin{lrbox}{\GrayRoundedBox}
		\begin{minipage}{\RoundedBoxWidth}}%
		{   \end{minipage}
	\end{lrbox}
	\begin{center}
		\begin{tikzpicture}%
			\node(Text)[draw=black!20,fill=white,rounded corners,%
			inner sep=2ex,text width=\RoundedBoxWidth]%
			{\usebox{\GrayRoundedBox}};
			\coordinate(x) at (current bounding box.north west);
			\node [draw=white,rectangle,inner sep=3pt,anchor=north west,fill=white] 
			at ($(x)+(6pt,.75em)$) {\boxheading};
		\end{tikzpicture}
\end{center}}     

\newenvironment{defproblemx}[2][]{\noindent\ignorespaces%
	\FrameSep=6pt%
	\parindent=0pt%
	\vspace*{-1.5em}
	\ifthenelse{\isempty{#1}}{%
		\begin{GrayBox}{#2}%                
		}{%
			\begin{GrayBox}{#2 parameterized by~{#1}}%  
			}
			\newcommand\Prob{Problem:}%
			\newcommand\Input{Input:}%                        
			\begin{tabular*}{\textwidth}{@{\hspace{.1em}} >{\itshape} p{1.8cm} p{0.8\textwidth} @{}}%        
			}{
			\end{tabular*}%
		\end{GrayBox}%
		\ignorespacesafterend
	}  
	
	\newcommand{\defparproblema}[4]{% FJR Version
		\begin{defproblemx}[#3]{#1}
			Input:  & #2 \\
			Task: & #4
		\end{defproblemx}
	}%
	
	\newcommand{\defparproblemanl}{\defparproblema}
	
	\newcommand{\defproblema}[3]{% FJR Version
		\begin{defproblemx}{#1}
			Input:  & #2 \\
			Task: & #3
		\end{defproblemx}
	}%
	
	%%%%%%%%%%%%%%%%%%%%%%%%
	\newcommand{\defproblemu}[3]{
		\vspace{1mm}
		\noindent\fbox{
			\begin{minipage}{0.95\textwidth}
				#1 \\
				{\bf{Input:}} #2  \\
				{\bf{Question:}} #3
			\end{minipage}
		}
		\vspace{1mm}
	}
	
	\newcommand{\defparproblem}[4]{
		\vspace{1mm}
		\noindent\fbox{
			\begin{minipage}{0.96\textwidth}
				\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
				{\bf{Input:}} #2  \\
				{\bf{Question:}} #4
			\end{minipage}
		}
		\vspace{1mm}
	}
	
	\newcommand{\defparproblemlist}[4]{
		\vspace{1mm}
		\noindent\fbox{
			\begin{minipage}{0.96\textwidth}
				\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
				{\bf{Input:}} #2  \\
				{\bf{Output:}} #4
			\end{minipage}
		}
		\vspace{1mm}
	}
	
	
	
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%
	\newcommand{\problemdef}[4]{
		\vspace{5mm} 
		\setlength{\fboxrule}{2pt}
		\noindent\fbox{
			\begin{minipage}{\textwidth}
				\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 
					\\ \end{tabular*}
				{\bf{Instance:}} #2  \\
				{\bf{Parameter:}} #3 \\
				{\bf{Question:}} #4
			\end{minipage}
		}
		\vspace{4mm}
	} 



